Bayesian Federated Learning with Hamiltonian Monte Carlo: Algorithm and Theory

This work introduces a novel and efficient Bayesian federated learning algorithm, namely, the Federated Averaging stochastic Hamiltonian Monte Carlo (FA-HMC), for parameter estimation and uncertainty quantification. We establish rigorous convergence guarantees of FA-HMC on non-iid distributed data sets, under the strong convexity and Hessian smoothness assumptions. Our analysis investigates the effects of parameter space dimension, noise on gradients and momentum, and the frequency of communication (between the central node and local nodes) on the convergence and communication costs of FA-HMC. Beyond that, we establish the tightness of our analysis by showing that the convergence rate cannot be improved even for continuous FA-HMC process. Moreover, extensive empirical studies demonstrate that FA-HMC outperforms the existing Federated Averaging-Langevin Monte Carlo (FA-LD) algorithm.

==> prooflemmas.tex <==
\section{Proof of preliminary lemmas}


%\Wei{what is $\bar\theta$, how it is defined?}
\subsection{Proof of Lemma \ref{lem:GuD3}}
\label{contraction_divergence}
Introduce an immediate variable $\bar{\theta}(t)$ which follows HMC system with initial position $\theta(0)$ and initial momentum $\widetilde{p}(0)$. Noting that $\cH_t\theta(0)-\cH_t\widetilde{\theta}(0)=\cH_t\theta(0)-\cH_t\bar{\theta}(0)+\cH_t\bar{\theta}(0)-\cH_t\widetilde{\theta}(0)$, by triangle's inequality
\[
\|\cH_t\theta(0)-\cH_t\widetilde{\theta}(0)\|_2\leq \|\cH_t\theta(0)-\cH_t\bar{\theta}(0)\|_2+\|\cH_t\bar{\theta}(0)-\cH_t\widetilde{\theta}(0)\|_2
\]
By Lemma 6 in \cite{chen2019optimal}, we immediately obtain $\|\cH_t\bar{\theta}(0)-\cH_t\widetilde{\theta}(0)\|_2\leq (1-\frac{\mu t^2}{4})\|\bar{\theta}(0)-\widetilde{\theta}_0\|_2=(1-\frac{\mu t^2}{4})\|\theta(0)-\widetilde{\theta}_0\|_2$. Therefore it suffices to show that
\begin{equation}\label{pflem:contra:1}
   \|\cH_t\theta(0)-\cH_t\bar{\theta}(0)\|_2\leq Ct\|p(0)-\widetilde{p}(0)\|_2. 
\end{equation}
By definitions and  elementary calculations
\[
|\frac{d\|p(t)-\bar{p}(t)\|_2}{dt}|%=\frac{1}{2\|p(t)-\bar{p}(t)\|_2}\frac{d\|p(t)-\bar{p}(t)\|_2^2}{dt}=-\frac{\langle \nabla f(x)\rangle}{}
\leq L\|\theta(t)-\bar{\theta}(t)\|_2.
\]
This gives
\[
\|p(t)-\bar{p}(t)\|_2\leq \|p(0)-\bar{p}(0)\|_2+\int_{0}^sL\|\theta(u)-\bar{\theta}(u)\|_2du
\]
and
\[
\|\theta(t)-\bar{\theta}(t)\|_2\leq \|\theta(0)-\bar{\theta}(0)\|_2+t\|p(0)-\bar{p}(0)\|_2+\int_0^t\int_{0}^sL\|\theta(u)-\bar{\theta}(u)\|_2duds
\]
By elementary ODE, we get
\[
\|\theta(t)-\bar{\theta}(t)\|_2\leq\|\theta(0)-\bar{\theta}(0)\|_2\cosh(\sqrt{L}t)+\frac{\|p(0)-\bar{p}(0)\|_2}{\sqrt{L}}\sinh (\sqrt{L}t),
\]
%\Wei{Double check, is it OK?}
where the first term in the RHS is $0$ since $\bar{\theta}(0)=\theta(0)$ and $\sinh (\sqrt{L}t)\leq C\sqrt{L}t$ for all $C>\sinh(0.5)$ and $0\leq \sqrt{Lt}\leq 0.5$. This proves (\ref{pflem:contra:1}) and finishes the proof of $(a)$.% \Wei{if this technique was devised by Chen's work, you may need to mention it a little bit, otherwise, it is not that clear.}

$(b)$ follows by applying Cauchy-Schwarz inequality on $(a)$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Lemma \ref{lem:longtermerror}}
Applying $(b)$ in Lemma \ref{lem:GuD3} recursively, we get
\begin{align}
\begin{split}\label{pf:lemlongterm:1}
        \|({\cal H}_u)^E (\theta)-({\cal H}_u)^E&(\theta^*)\|_{2}^2 \\
        \leq &(1+\beta)(1-\frac{\mu}{4}u^2) \|(\cH_u)^{E-1}(\theta)-(\cH_u)^{E-1}(\theta^*)\|_2^2+(1+\frac{1}{\beta})C^2u^2\|p_{E-1}\|_2^2 \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq & \cdots \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq &\Bigl[(1+\beta)(1-\frac{\mu}{4}u^2)\Bigr]^E \|\theta-\theta^*\|_2^2+\sum_{j=1}^E[(1+\beta) (1-\frac{\mu}{4}u^2)]^{E-j}(1+\frac{1}{\beta})C^2u^2\|p_{j-1}\|_2^2.
\end{split}
\end{align}
Set $\beta=\mu u^2/(4-\mu u^2$ and so $(1+\beta)(1-\frac{\mu}{4}u^2)=1$, $1+\frac{1}{\beta}\leq \frac{4}{\mu u^2}$,  we get the result for the first claim.
%No better than the first
%For the second claim, we can set $\beta= \frac{E^{1/E}}{1-\mu u^2/4}-1$ and so 
%\[
%(1+\beta)(1-\frac{\mu}{4}u^2)=E^{\frac{1}{E}},\qquad 1+\frac{1}{\beta}=\frac{E^{\frac{1}{E}}}{E^{\frac{1}{E}}-1+\mu u^2/4}\leq \frac{C_0^{1/C_0}}{C_0^{1/C_0}-1},
%\]
%where we have used that $x^{1/x}\geq C_0^{1/C_0}$ if $1<x\leq C_0$.

%Putting these into (\ref{pf:lemlongterm:1}) gives 
%\begin{align*}
%   \|({\cal H}_u)^E (\theta)-({\cal H}_u)^E(\theta^*)\|_{2}^2 \leq & E  \|\theta-\theta^*\|_2^2+\sum_{j=1}^EE^{1-j/E}\frac{C_0^{1/C_0}}{C_0^{1/C_0}-1}C^2u^2\|p_{j-1}\|_2^2
%\end{align*}
Note that $E^{1/j/E}\leq E$, the second claim follows.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma \ref{lem:diffHMCs}}
\iffalse
By triangle's inequality
\begin{equation}\label{pf:lem:dis:1}
    \|\sum_{c=1}^Nw_c\cH^{(c),i+1}_{K\eta_t}(\theta^{\pi})-\cH^{\pi,i+1}_{K\eta_t}(\theta^{\pi})\|_2^2\leq (1+\alpha)(I)+(1+\frac{1}{\alpha})(II),
\end{equation}
where
\begin{align*}
    (I)&:\Bigl\|\cH^{\pi}_{K\eta_t}\Bigl(\sum_{c=1}^Nw_c\cH^{(c),i}_{K\eta_t}(\theta^{\pi})\Bigr)-\cH^{\pi,i+1}_{K\eta_t}(\theta^{\pi})\Bigr\|_2^2\\
    (II)&:\Bigl\|\sum_{c=1}^Nw_c\cH^{(c),i+1}_{K\eta_t}(\theta^{\pi})-\cH^{\pi}_{K\eta_t}\Bigl(\sum_{c=1}^Nw_c\cH^{(c),i}_{K\eta_t}(\theta^{\pi})\Bigr)\Bigr\|_2^2
\end{align*}
Consider $(I)$. By Lemma \ref{lem:conb},
\begin{equation}\label{pf:lem:dis:2}
  \mathbb{E}[(I)]\leq (1-\frac{\mu(K\eta_t)^2}{4})\mathbb{E}\Bigl[\Bigl\|\sum_{c=1}^Nw_c\cH^{(c),i}_{K\eta_t}(\theta^{\pi})-\cH^{\pi,i}_{K\eta_t}(\theta^{\pi})\Bigr\|_2^2\Bigr].  
\end{equation}
Consider $(II)$. Let $\theta_{\pi}^{(c),i}(u)$ and $\bar{\theta}^{\pi}(u)$ denote $\cH^{(c)}_u(\cH^{(c),i}(\theta^{\pi}))$ and $\cH^{\pi}_u(\sum_{c=1}^Nw_c\cH^{(c),i}(\theta^{\pi}))$ respectively, for any $u\in [0,K\eta_t]$%Let $q^{(c)}(u)$ be the position at time $u$ following the $c$-th HMC system $\cH^{(c)}$ with initial position $\cH^{(c),i}_{K\eta_t}(\theta^{\pi})$ and initial momentum $p_i$ and let $q^{\pi}(u)$ be the position at time $u$ following the  HMC system $\cH$ with initial position $\cH^{(c),i}_{K\eta_t}(\theta^{\pi})$ and initial momentum $p_i$.  

By definitions and direct calculations,
\begin{align*}
    (II)=&\Bigl\|0-\sum_{c=1}^Nw_c\int_0^{K\eta_t}\int_0^s \Bigl(\nabla f^{(c)}(\theta_{\pi}^{(c),i}(u))-\nabla f^{(c)}(\bar{\theta}^{\pi}(u) )\Bigr)duds\Bigr\|_2^2\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq & \sum_{c=1}^Nw_c\Bigl\|\int_0^{K\eta_t}\int_0^s\Bigl(\nabla f^{(c)}(\theta_{\pi}^{(c),i}(u))-\nabla f^{(c)}(\bar{\theta}^{\pi}(u) )\Bigr)duds\Bigr\|_2^2\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq & \sum_{c=1}^Nw_c\frac{(K\eta_t)^2}{2}\int_0^{K\eta_t}\int_0^s\|\nabla f^{(c)}(\theta_{\pi}^{(c),i}(u))-\nabla f^{(c)}(\bar{\theta}^{\pi}(u) )\|_2^2duds\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq & \sum_{c=1}^Nw_c\frac{(K\eta_t)^2}{2}\int_0^{K\eta_t}\int_0^sL^2\|\theta_{\pi}^{(c),i}(u)-\bar{\theta}^{\pi}(u) \|_2^2duds\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \leq & \sum_{c=1}^Nw_c\frac{(K\eta_t)^2L^2}{2}\int_0^{K\eta_t}\int_0^s3(\|\theta_{\pi}^{(c),i}(u)-\theta^{\pi(c),i}(u)\|_2^2+\|\theta^{\pi(c),i}(u)-\theta^{\pi,i}(u)\|_2^2\\
            &+\|\theta^{\pi,i}(u)-\bar{\theta}^{\pi}(u) \|_2^2)duds
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{align*}
where the first inequality is by convexity of $\|\cdot\|_2^2$; the second inequality and the fourth inequality are by Cauchy-Schwarz inequality; the third inequality is by the smoothness assumption \ref{assum:smooth}.


At the same time, by Lemma \ref{lem:GuD3},
\begin{align*}
    \|\theta_{\pi}^{(c),i}(u)-\theta^{\pi(c),i}(u)\|_2^2\leq & (1-\frac{\mu u^2}{4})(1-\frac{\mu(K\eta_t)^2}{4})^i\|\theta^{\pi}-\theta^{\pi(c)}\|_2^2\leq \|\theta^{\pi}-\theta^{\pi(c)}\|_2^2\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \|\theta^{\pi,i}(u)-\bar{\theta}^{\pi}(u) \|_2^2\leq& \|\theta^{\pi,i}-\bar{\theta}^{\pi} \|_2^2:=\|\theta^{\pi,i}-\sum_{c=1}^Nw_c\cH^{(c),i}(\theta^{\pi})\|_2^2
\end{align*}
and by convexity and triangle's inequality,
\begin{align*}
   \|\theta^{\pi,i}-\sum_{c=1}^Nw_c\cH^{(c),i}(\theta^{\pi})\|_2^2\leq& 2\sum_{c=1}^Nw_c\Bigl( \|\theta^{\pi,i}-\theta^{\pi(c),i}\|_2^2+  \|\theta^{\pi(c),i}-\cH^{(c),i}(\theta^{\pi})\|_2^2\Bigr)\\
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \leq& 2\sum_{c=1}^Nw_c\Bigl( \|\theta^{\pi,i}-\theta^{\pi(c),i}\|_2^2+  \|\theta^{\pi(c)}-\theta^{\pi}\|_2^2\Bigr).
\end{align*}
Combining these, we got
\begin{align*}
    \mathbb{E}[(II)]\leq & \sum_{c=1}^Nw_c3(K\eta_t)^4L^2\mathbb{E}\Bigl[\|\theta^{\pi}-\theta^*\|^2+\|\theta^*-\theta^{*(c)}\|^2+\|\theta^{*(c)}-\theta^{\pi(c)}\|_2^2\Bigr]\\
    \leq& (K\eta_t)^4L^2\Bigl(\frac{d}{\mu}+\sum_{c=1}^Nw_c\|\theta^*-\theta^{*(c)}\|^2\Bigr)
\end{align*}
and so
\begin{align*}
    \mathbb{E}\|\sum_{c=1}^Nw_c\cH^{(c),i+1}_{K\eta_t}(\theta^{\pi})-\cH^{\pi,i+1}_{K\eta_t}(\theta^{\pi})\|_2^2\leq & (1+\alpha)(1-\frac{\mu(K\eta_t)^2}{4})\mathbb{E}\|\sum_{c=1}^Nw_c\cH^{(c),i}_{K\eta_t}(\theta^{\pi})-\cH^{\pi,i}_{K\eta_t}(\theta^{\pi})\|_2^2\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  &+(1+\frac{1}{\alpha})(K\eta_t)^4L^2\Bigl(\frac{d}{\mu}+\sum_{c=1}^Nw_c\|\theta^*-\theta^{*(c)}\|^2\Bigr).  
\end{align*}
Setting $(1+\alpha)(1-\frac{\mu(K\eta_t)^2}{4})=(1-\frac{\mu(K\eta_t)^2}{8})$, and by induction,
\[
\mathbb{E}\|\sum_{c=1}^Nw_c\cH^{(c),i+1}_{K\eta_t}(\theta^{\pi})-\cH^{\pi,i+1}_{K\eta_t}(\theta^{\pi})\|_2^2\leq \frac{64L^2}{\mu^2}\Bigl(\frac{d}{\mu}+\sum_{c=1}^Nw_c\|\theta^*-\theta^{*(c)}\|^2\Bigr).  
\]
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
By triangle's inequality and  convexity
\begin{align*}
    \|\sum_{c=1}^Nw_c\theta_{\pi}^{(c),i}-\theta^{\pi,i}\|^2\leq& 2 \Bigl(\|\sum_{c=1}^Nw_c\theta_{\pi}^{(c),i}-\sum_{c=1}^Nw_c\theta^{\pi(c),i}\|^2+\|\sum_{c=1}^Nw_c\theta^{\pi(c),i}-\theta^{\pi,i}\|^2\Bigr)\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq &2 \sum_{c=1}^Nw_c\Bigl(\|\theta_{\pi}^{(c),i}-\theta^{\pi(c),i}\|^2+\|\theta^{\pi(c),i}-\theta^{\pi,i}\|^2\Bigr)
\end{align*}
At the same time, by   Lemma \ref{lem:GuD3}
\begin{align*}
  \|\theta_{\pi}^{(c),i}-\theta^{\pi(c),i}\|^2\leq (1-\frac{\mu(K\eta_t)^2}{4})^i\|\theta^{\pi}-\theta^{\pi(c)}\|^2
  \leq \|\theta^{\pi}-\theta^{\pi(c)}\|^2.
\end{align*}
We have
\[
\mathbb{E}[\|\sum_{c=1}^Nw_c\theta_{\pi}^{(c),i}-\theta^{\pi,i}\|^2]\leq 4 \sum_{c=1}^Nw_c\mathbb{E}\Bigl(\|\theta^{\pi}-\theta^*\|^2+\|\theta^*-\theta^{*(c)}\|^2+\|\theta^{*(c)}-\theta^{\pi(c)}\|^2\Bigr)\leq 4(\frac{2d}{\mu}+\sum_{c=1}^Nw_c\|\theta^*-\theta^{*(c)}\|^2).
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\subsection{Proof of Lemma \ref{lem:difftHMCs}}
Introduce an intermediate HMC system $\bar{\theta}(t)=\widetilde{{\cal H}}_t(\bar{\theta}(0))$ with initial position $\bar{\theta}(0)=\theta(0)$ and initial momentum $\bar{p}(0)=p(0)$. By Cauchy-Schwarz inequality, for any $\alpha>0$
\begin{equation}\label{pflem:difftHMCs:1}
    \|{\cal H}_t \theta(0)-\widetilde{{\cal H}}_t \widetilde{\theta}(0)\|_{2}^2=(1+\frac{1}{\alpha})\|{\cal H}_t \theta(0)-\widetilde{{\cal H}}_t(\bar{\theta}(0))\|^2+(1+\alpha)\|\widetilde{{\cal H}}_t(\bar{\theta}(0))-\widetilde{{\cal H}}_t \widetilde{\theta}(0)\|_2^2,
\end{equation}
where by Lemma \ref{lem:GuD3} and $(\bar{\theta}(0),\bar{p}(0))=(\theta(0),p(0))$
\begin{equation}\label{pflem:difftHMCs:2}
   \|\widetilde{{\cal H}}_t(\bar{\theta}(0))-\widetilde{{\cal H}}_t \widetilde{\theta}(0)\|_2\leq (1-\frac{\mu}{4}t^2)\|\bar{\theta(0)}-\widetilde{\theta}(0)\|_{2}+Ct\|\bar{p}(0)-\widetilde{p}(0)\|_{2}\equiv \Delta. 
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
At the same time, by direct calculations
\begin{align}
\begin{split}\label{pflem:difftHMCs:3}
     \|{\cal H}_t \theta(0)-\widetilde{{\cal H}}_t(\bar{\theta}(0))\|_2=&\|{\cal H}_t \theta(0)-\theta^*+\theta^*-\widetilde{\theta}^*+\widetilde{\theta}^*-\widetilde{{\cal H}}_t(\bar{\theta}(0))\|_2\\
\leq & \|{\cal H}_t \theta(0)-\theta^*\|_2+\|\theta^*-\widetilde{\theta}^*\|_2+\|\widetilde{\theta}^*-\widetilde{{\cal H}}_t(\bar{\theta}(0))\|_2  \\
\leq & \|\theta(0)-\theta^*\|_2+Ct\|p(0)\|_2+\|\theta^*-\widetilde{\theta}^*\|_2+\|\theta(0)-\widetilde{\theta}^*\|_2+Ct\|p(0)\|_2\\
\leq &2\|\theta(0)-\theta^*\|_2+2Ct\|p(0)\|_2+2\|\theta^*-\widetilde{\theta}^*\|_2. 
\end{split}
\end{align}
where the first inequality is by triangle's inequality; the second inequality is by Lemma \ref{lem:GuD3} and noting that ${\cal H}_t(\theta^*,0)=(\theta^*,0)$ and $\widetilde{{\cal H}}_t(\theta^*,0)=(\theta^*,0)$; the last inequality is by triangle's inequality $\|\theta(0)-\widetilde{\theta}^*\|_2\leq \|\theta(0)-\theta^*\|_2+\|\theta^*-\widetilde{\theta}^*\|_2$.

Combining (\ref{pflem:difftHMCs:1})-(\ref{pflem:difftHMCs:3}) finishes the proof.
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Lemma \ref{lem:ubound}}
\begin{proof}
The claim $(c)$ and $(d)$ follow directly from $(a)$ and $(b)$ by summing over weights $w_c$, $c=1,2,\ldots,N$. We only proves $(a)$ and $(b)$ below.

Consider $(a)$ first. By triangle's inequality, for any $\alpha_t>0$
\begin{align}\label{pflem:ubound:1}
\begin{split}
             \|\theta^{(c),i}_t(u)-\theta^{\pi,Et+i}_{\pi}(u)\|^2 =& \|\theta^{(c),i}_t(u)-\cH^{(c)}_u(\theta^{\pi,Et+i}_{\pi})+\cH^{(c)}_u(\theta^{\pi,Et+i}_{\pi})-\theta^{\pi,Et+i}_{\pi}(u)\|^2\\
            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
             \leq&  (1+\alpha_t)(I) +(1+\frac{1}{\alpha_t})(II),
\end{split}
\end{align}
where 
\[
(I)=\|\theta^{(c),i}_t(u)-\cH^{(c)}_u(\theta^{\pi,Et+i}_{\pi}))\|^2,\qquad (II)=\|\cH^{(c)}_u(\theta^{\pi,Et+i}_{\pi}))-\theta^{\pi,Et+i}_{\pi}(u)\|^2.
\]
Consider $(I)$, by Lemma \ref{lem:GuD3},
\begin{equation}\label{pflem:ubound:2}
    (I)\leq (1-\frac{\mu u^2}{4})\|\theta^{(c),i}_t-\theta^{\pi,Et+i}_{\pi}\|^2
\end{equation}
Next consider $(II)$, by definitions
\begin{align*}
 (II)=&\Bigl\|\int_{0}^u\int_0^s\Bigl(\nabla f^{(c)}(\cH^{(c)}_r(\theta^{\pi,Et+i}_{\pi}))-\nabla f(\theta^{\pi,Et+i}_{\pi}(r))\Bigr)drds\Bigr\|^2   \\
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \leq &\frac{u^2}{2}\int_{0}^u\int_0^s\|\nabla f^{(c)}(\cH^{(c)}_r(\theta^{\pi,Et+i}_{\pi}))-\nabla f(\theta^{\pi,Et+i}_{\pi}(r))\|^2drds \\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 = &\frac{u^2}{2}\int_{0}^u\int_0^s\|\nabla f^{(c)}(\cH^{(c)}_r(\theta^{\pi,Et+i}_{\pi}))-\nabla f^{(c)}(\theta^{*(c)})+\nabla f(\theta^*)-\nabla f(\theta^{\pi,Et+i}_{\pi}(r))\|^2drds \\
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \leq &u^2\int_{0}^u\int_0^s(\|\nabla f^{(c)}(\cH^{(c)}_r(\theta^{\pi,Et+i}_{\pi}))-\nabla f^{(c)}(\theta^{*(c)})\|^2+\|\nabla f(\theta^*)-\nabla f(\theta^{\pi,Et+i}_{\pi}(r))\|^2)drds \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \leq &u^2L^2\int_{0}^u\int_0^s(\|\cH^{(c)}_r(\theta^{\pi,Et+i}_{\pi})-\theta^{*(c)}\|^2+\|\theta^*-\theta^{\pi,Et+i}_{\pi}(r))\|^2)drds \\
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \leq &u^2L^2\int_{0}^u\int_0^s(2\|\cH^{(c)}_r(\theta^{\pi,Et+i}_{\pi})-\theta^{\pi(c),Et+i}_{\pi(c)}(r)\|^2+2\|\theta^{\pi(c),Et+i}_{\pi(c)}(r)-\theta^{*(c)}\|^2+\|\theta^*-\theta^{\pi,Et+i}_{\pi}(r))\|^2)drds \\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \leq &u^2L^2\int_{0}^u\int_0^s(2\|\theta^{\pi,Et+i}_{\pi}-\theta^{\pi(c),Et+i}_{\pi(c)}\|^2+2\|\theta^{\pi(c),Et+i}_{\pi(c)}(r)-\theta^{*(c)}\|^2+\|\theta^*-\theta^{\pi,Et+i}_{\pi}(r))\|^2)drds \\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \leq &u^2L^2\int_{0}^u\int_0^s(6(\|\theta^{\pi,Et+i}_{\pi}-\theta^*\|^2+\|\theta^*-\theta^{*(c)}\|^2+\|\theta^{*(c)}-\theta^{\pi(c),Et+i}_{\pi(c)}\|^2)\\
  &\hspace{2cm}+2\|\theta^{\pi(c),Et+i}_{\pi(c)}(r)-\theta^{*(c)}\|^2+\|\theta^*-\theta^{\pi,Et+i}_{\pi}(r))\|^2)drds,
\end{align*}
where the first, second, fourth and sixth inequality are by Cauchy-Schwarz inequality; the second equality is by that $\theta^{*(c)}$ and $\theta^*$ are the maximizer of $f^{(c)}$ and $l$, respectively and so  $\nabla f^{(c)}(\theta^{*(c)})=\nabla f(\theta^*)=0$;  the third inequality is by the smoothness assumption \ref{assum:smooth}.

Further taking expectation on both sides and by Lemma \ref{lem:Oracle} 
\begin{equation} \label{pflem:ubound:3}
    \mathbb{E}(II)\leq u^2L^2\int_{0}^u\int_0^s(6(\frac{d}{\mu}+\|\theta^*-\theta^{*(c)}\|^2+\frac{d}{\mu})+2\frac{d}{\mu}+\frac{d}{\mu})drds =u^4L^2(\frac{15d}{2\mu}+3\|\theta^*-\theta^{*(c)}\|^2).
\end{equation}
Combining (\ref{pflem:ubound:1})-(\ref{pflem:ubound:3}) give that for any $\alpha_t>0$
\[
      \mathbb{E} \|\theta^{(c),i}_t(u)-\theta^{\pi,Et+i}_{\pi}(u)\|^2 \leq (1+\alpha_t) (1-\frac{\mu u^2}{4})\mathbb{E}\|\theta^{(c),i}_t-\theta^{\pi,Et+i}_{\pi}\|^2+(1+\frac{1}{\alpha_t})u^4L^2(\frac{15d}{2\mu}+3\|\theta^*-\theta^{*(c)}\|^2).
\]
Set $(1+\alpha_t)(1-\frac{\mu (K\eta_t)^2}{4})=(1-\frac{\mu (K\eta_t)^2}{8})$  (so $1+\frac{1}{\alpha_t}=\frac{8-\mu (K\eta_t)^2}{\mu (K\eta_t)^2)}\leq \frac{8(K\eta_t)^2}{\mu u^4}$) with $u\leq K\eta_t$ gives
\begin{equation}\label{pflem:ubound:4}
      \mathbb{E} \|\theta^{(c),i}_t(u)-\theta^{\pi,Et+i}_{\pi}(u)\|^2 \leq (1-\frac{\mu (K\eta_t)^2}{8})\mathbb{E}\|\theta^{(c),i}_t-\theta^{\pi,Et+i}_{\pi}\|^2+\frac{8(K\eta_t)^2L^2}{\mu}(\frac{15d}{2\mu}+3\|\theta^*-\theta^{*(c)}\|^2).
\end{equation}
Set $u=K\eta_t$ and note that $(\theta^{(c),i+1}_t,\theta^{\pi,Et+i+1}_{\pi})=(\theta^{(c),i}_t(K\eta_t),\theta^{\pi,Et+i}(K\eta_t))$ and that  $\theta^{(c),0}_t=\theta_t$, for any $c=1,2,\ldots,N$.
\begin{align*}
\mathbb{E} \|\theta^{(c),i+1}_t-\theta^{\pi,Et+i+1}_{\pi}\|^2 \leq& (1-\frac{\mu (K\eta_t)^2}{8})\mathbb{E}\|\theta^{(c),i}_t-\theta^{\pi,Et+i}_{\pi}\|^2+\frac{8(K\eta_t)^2L^2}{\mu}(\frac{15d}{2\mu}+3\|\theta^*-\theta^{*(c)}\|^2)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\leq & \cdots \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\leq & (1-\frac{\mu (K\eta_t)^2}{8})^{i+1}\mathbb{E}\|\theta^{(c),0}_t-\theta^{\pi,Et}_{\pi}\|^2\\
&+\sum_{j=0}^i(1-\frac{\mu (K\eta_t)^2}{8})^j\frac{8(K\eta_t)^2}{\mu}L^2(\frac{15d}{2\mu}+3\|\theta^*-\theta^{*(c)}\|^2)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\leq & (1-\frac{\mu (K\eta_t)^2}{8})^{i+1}\mathbb{E}\|\theta_t-\theta^{\pi,Et}_{\pi}\|^2\\
&+\sum_{j=0}^i(1-\frac{\mu (K\eta_t)^2}{8})^j\frac{8(K\eta_t)^2}{\mu}L^2(\frac{15d}{2\mu}+3\|\theta^*-\theta^{*(c)}\|^2)
\end{align*}
Note that $\theta_{t+1}\sum_{c=1}^Nw_c\theta^{(c),E}_t$ for $t=0,1,\ldots$, by convexity of $\|\cdot\|^2$ we further have 
\begin{align*}
    \mathbb{E} \|\theta_{t+1}-\theta^{\pi}_{t+1}\|^2\leq &  \sum_{c=1}^Nw_c\mathbb{E} \|\theta^{(c),E}_t-\theta^{\pi,Et+E}_{\pi}\|^2\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq & \cdots \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq & (1-\frac{\mu (K\eta_t)^2}{8})^E\sum_{c=1}^Nw_c\mathbb{E}\|\theta^{(c),0}_t-\theta^{\pi,Et}_{\pi}\|^2\\
&+\sum_{j=0}^E(1-\frac{\mu (K\eta_t)^2}{8})^j\frac{8(K\eta_t)^2}{\mu}L^2(\frac{15d}{2\mu}+3\sum_{c=1}^Nw_c\|\theta^*-\theta^{*(c)}\|^2)\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    = & (1-\frac{\mu (K\eta_t)^2}{8})^E\mathbb{E}\|\theta_t-\theta^{\pi,Et}_{\pi}\|^2\\
&+\sum_{j=0}^E(1-\frac{\mu (K\eta_t)^2}{8})^j\frac{8(K\eta_t)^2}{\mu}L^2(\frac{15d}{2\mu}+3\sum_{c=1}^Nw_c\|\theta^*-\theta^{*(c)}\|^2)
\end{align*}
By induction,
\begin{align*}
  \mathbb{E} \|\theta_t-\theta^{\pi,Et}_{\pi}\|^2\leq &(1-\frac{\mu (K\eta_t)^2}{8})^{Et}\mathbb{E}\|\theta_0-\theta^\pi\|^2\\
  &+\sum_{j=0}^{Et-1}(1-\frac{\mu (K\eta_t)^2}{8})^j\frac{8(K\eta_t)^2L^2}{\mu}(\frac{15d}{2\mu}+3\sum_{c=1}^Nw_c\|\theta^*-\theta^{*(c)}\|^2)
\end{align*}
Combining the above  gives
\begin{align*}
    &\mathbb{E} \|\theta^{(c),i}_t(u)-\theta^{\pi,Et+i}_{\pi}(u)\|^2\\
    \leq &(1-\frac{\mu (K\eta_t)^2}{8})\mathbb{E}\|\theta^{(c),i}_t-\theta^{\pi,Et+i}_{\pi}\|^2+\frac{8(K\eta_t)^2L^2}{\mu}(\frac{15d}{2\mu}+3\|\theta^*-\theta^{*(c)}\|^2)\\
    \leq & (1-\frac{\mu (K\eta_t)^2}{8})^{i+1}\mathbb{E}\|\theta_t-\theta^{\pi,Et}_{\pi}\|^2+\sum_{j=0}^i(1-\frac{\mu (K\eta_t)^2}{8})^j\frac{8(K\eta_t)^2L^2}{\mu}(\frac{15d}{2\mu}+3\|\theta^*-\theta^{*(c)}\|^2)\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq &(1-\frac{\mu (K\eta_t)^2}{8})^{Et+i+1}\mathbb{E}\|\theta_0-\theta^{\pi}\|^2+\sum_{j=i+1}^{Et}(1-\frac{\mu (K\eta_t)^2}{8})^j\frac{8(K\eta_t)^2L^2}{\mu}(\frac{15d}{2\mu}+3\sum_{c=1}^Nw_c\|\theta^*-\theta^{*(c)}\|^2)\\
    &+\sum_{j=0}^i(1-\frac{\mu (K\eta_t)^2}{8})^j\frac{8(K\eta_t)^2L^2}{\mu}(\frac{15d}{2\mu}+3\|\theta^*-\theta^{*(c)}\|^2)\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq & \mathbb{E}\|\theta_0-\theta^{\pi}\|^2+\frac{32L^2}{\mu^2}\Bigl(15\frac{d}{\mu}+6(1-m)\|\theta^*-\theta^{*(c)}\|^2+6m\sum_{c=1}^Nw_c\|\theta^*-\theta^{*(c)}\|^2\Bigr),
\end{align*}
where $m=(1-\frac{\mu (K\eta_t)^2}{8})^{i+1})$. Note that $(1-\frac{\mu (K\eta_t)^2}{8})^{Et+i+1}\leq 1$, this proves $(a)$.

Consider $(b)$. Note that
\begin{align*}
    \mathbb{E}\|\nabla f^{(c)}(\theta^{(c),i}_t(u))\|^2=&\mathbb{E}\|\nabla f^{(c)}(\theta^{(c),i}_t(u))-\nabla f^{(c)}(\theta^{*(c)}\|^2\\
    \leq &L^2\mathbb{E}\|\theta^{(c),i}_t(u)-\theta^{*(c)}\|^2\\
    \leq &3L^2 (\mathbb{E}\|\theta^{(c),i}_t(u)-\theta^{\pi,Et+i}_{\pi}(u)\|^2+\mathbb{E}\|\theta^{\pi,Et+i}_{\pi}(u)-\theta^*\|^2+\|\theta^*-\theta^{*(c)}\|^2)
\end{align*}
where the first inequality is by the smoothness assumption \ref{assum:smooth}; the second inequality is by Cauchy-Schwarz inequality. Applying $(a)$ on $\mathbb{E}\|\theta^{(c),i}_t(u)-\theta^{\pi,Et+i}_{\pi}(u)\|^2$ and Lemma \ref{lem:Oracle} on $\mathbb{E}\|\theta^{\pi,Et+i}_{\pi}(u)-\theta^*\|^2$ gives
\begin{align*}
  \mathbb{E}\|\nabla f^{(c)}(\theta^{(c),i}_t(u))\|^2
    \leq & 3L^2 (\mathbb{E}\|\theta_0-\theta^{\pi}\|^2+\frac{32L^2}{\mu^2}\Bigl(15\frac{d}{\mu}+6(1-m)\|\theta^*-\theta^{*(c)}\|^2\\
    &+6m\sum_{c=1}^Nw_c\|\theta^*-\theta^{*(c)}\|^2\Bigr)+\frac{d}{\mu}+\|\theta^*-\theta^{*(c)}\|^2)  
\end{align*}
This finishes the proof of $(b)$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Proof of Lemma \ref{lem:lbound}}
\lemlbound*
\begin{proof}
\begin{align*}
    \sum_{c=1}^Nw_c\|\cH^{(c),i}(\theta_t)-\sum_{j=1}^N&w_j\cH^{(j),i}(\theta_t)\|^2=\sum_{c=1}^Nw_c\Bigl\|(1-w_c)\Bigl(\cH^{(c),i}(\theta_t)-\theta_t\Bigr)-\sum_{j\neq c}w_j\Bigl(\cH^{(j),i}(\theta_t)-\theta_t\Bigr)\Bigr\|^2\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq &\sum_{c=1}^Nw_c(1-w_c+\sum_{j\neq c}w_j)\Bigl((1-w_c)\|\cH^{(c),i}(\theta_t)-\theta_t\|^2+\sum_{j\neq c}w_j\|\cH^{(j),i}(\theta_t)-\theta_t\|^2\Bigr)\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    =&\sum_{c=1}^Nw_c(1-w_c)\|\cH^{(c),i}(\theta_t)-\theta_t\|^2
\end{align*}
Next we bound $\|\cH^{(c),i}(\theta_t)-\theta_t\|^2$. By definitions,
\begin{align*}
    \mathbb{E}[\|\cH^{(c),i}(\theta_t)-\theta_t\|^2=&\|\sum_{j=1}^ip_j(K\eta_t)-\sum_{j=1}^i\int_0^{K\eta_t}\int_0^s\nabla f^{(c)}(\theta^{(c),j}_t(u))duds\|^2]\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq & (i+1)\mathbb{E}\Bigl(\|\sum_{j=1}^ip_j(K\eta_t)\|^2+\sum_{j=1}^i\|\int_0^{K\eta_t}\int_0^s\nabla f^{(c)}(\theta^{(c),j}_t(u))duds\|^2\Bigr)\\
    \leq &(i+1)\Bigl(id(K\eta_t)^2+\sum_{j=1}^i\frac{(K\eta_t)^2}{2}\int_0^{K\eta_t}\int_0^s\mathbb{E}\|\nabla f^{(c)}(\theta^{(c),j}_t(u))\|^2duds\Bigr)\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq &E^2(K\eta_t)^2(d+\frac{(K\eta_t)^2B}{4}),
\end{align*}
where the last inequality is by Lemma \ref{lem:ubound}.

The claim follows by combining the above and that $\sum_{c=1}^Nw_c(1-w_c)\leq \sum_{c=1}^Nw_c=1$.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

